An Empirical Investigation of Randomized Defenses against Adversarial Attacks

In recent years, Deep Neural Networks (DNNs) have had a dramatic impact on a variety of problems that were long considered very difficult, e. g., image classification and automatic language translation to name just a few. The accuracy of modern DNNs in classification tasks is remarkable indeed. At the same time, attackers have devised powerful methods to construct specially-crafted malicious inputs (often referred to as adversarial examples) that can trick DNNs into mis-classifying them. What is worse is that despite the many defense mechanisms proposed to protect DNNs against adversarial attacks, attackers are often able to circumvent these defenses, rendering them useless. This state of affairs is extremely worrying, especially since machine learning systems get adopted at scale. In this paper, we propose a scientific evaluation methodology aimed at assessing the quality, efficacy, robustness and efficiency of randomized defenses to protect DNNs against adversarial examples. Using this methodology, we evaluate a variety of defense mechanisms. In addition, we also propose a defense mechanism we call Randomly Perturbed Ensemble Neural Networks (RPENNs). We provide a thorough and comprehensive evaluation of the considered defense mechanisms against a white-box attacker model, six different adversarial attack methods and using the ILSVRC2012 validation data set.

==> figures/robu-overview.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[baseline]
        %%% FIRST LEFT %%%
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            %xlabel={$n$},
            ymin=0,
            ymax=0.4,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
        ]
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_99settings.csv};
        \end{axis}
    \end{tikzpicture}
    %%% FIRST RIGHT %%%
    \begin{tikzpicture}[baseline]
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            %xlabel={$n$},
            ymin=0,
            ymax=0.4,
            yticklabel pos=upper,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
            legend style={font=\scriptsize},
            legend entries={
                $\robustness{0.50}{n}$,
                $\robustness{0.80}{n}$,
                $\robustness{0.95}{n}$,
                $\robustness{0.99}{n}$,
                $\robustness{1.00}{n}$
            },
        ]
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_dfa_98settings.csv};
        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}[baseline]
        %%% SECOND LEFT %%%
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            %xlabel={$n$},
            ymin=0.0,
            ymax=0.4,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
        ]
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_99settings.csv};
        \end{axis}
    \end{tikzpicture}
    %%% SECOND RIGHT %%%
    \begin{tikzpicture}[baseline]
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            %xlabel={$n$},
            ymin=0,
            ymax=0.4,
            yticklabel pos=upper,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
        ]
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_cwl2_98settings.csv};
        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}[baseline]
        %%% THIRD LEFT %%%
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            %xlabel={$n$},
            ymin=0,
            ymax=0.4,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
        ]
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_99settings.csv};
        \end{axis}
    \end{tikzpicture}
    %%% THIRD RIGHT %%%
    \begin{tikzpicture}[baseline]
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            %xlabel={$n$},
            ymin=0,
            ymax=0.4,
            yticklabel pos=upper,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
        ]
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_98settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_linfbia_98settings.csv};
        \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}[baseline]
        %%% FOURTH LEFT %%%
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            xlabel={$n$},
            ymin=0.5,
            ymax=1,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
        ]
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_99settings.csv};
            \addplot+[mark options={scale=0.5}]table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_99settings.csv};
        \end{axis}
    \end{tikzpicture}
    %%% FOURTH RIGHT %%%
    \begin{tikzpicture}[baseline]
        \begin{axis}[
            width=0.55\columnwidth,
            height=0.20\textheight,
            xmode=log,
            log basis x={2},
            log ticks with fixed point,% Turn 2^1.00, 2^2.00, ... to 2, 4, ...
            xlabel={$n$},
            ymin=0.5,
            ymax=1,
            yticklabel pos=upper,
            y tick label style={
                /pgf/number format/.cd,
                    fixed,
                    precision=1,
                /tikz/.cd
            },
        ]
            \addplot+[mark options={scale=0.5}] table [x=n,y=0.5-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_98settings.csv};
            \addplot+[mark options={scale=0.5}] table [x=n,y=0.8-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_98settings.csv};
            \addplot+[mark options={scale=0.5}] table [x=n,y=0.95-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_98settings.csv};
            \addplot+[mark options={scale=0.5}] table [x=n,y=0.99-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_98settings.csv};
            \addplot+[mark options={scale=0.5}] table [x=n,y=1-robustness] {data/robustness/robustness_of_pwg_on_vgg19_lbfgs_98settings.csv};
        \end{axis}
    \end{tikzpicture}
    
    \caption{
        Estimated $\robuvar(\text{\dmnamesing}, \robulevel, \ninstalls)$ using $(\reldev, \esbsize) = (0.05, 7)$ (left graphs) and $(\reldev, \esbsize) = (0.11, 63)$ (right graphs) evaluated against the AE generation methods \AEMdfa\ (first row), \AEMcwltwo\ (second row), \AEMbimlinf\ (third row) and \AEMlbfgs\ (fourth row).
        Generally, lower values on the $y$-axis are preferable.
        Ideally they approach 0 as $n$ increases.
        Note that the $x$-axes for right hand side graphs just range up to 64 (compared to 256 on the left hand side) and scale on a logarithmic scale (base 2).
        Also note that the bottom graphs’ $y$-axes range from 0.5 to 1.0
        (in contrast to the other graphs’ $y$-axes).
    }
    \label{fig:robu-overview}
\end{figure}
